Measure of Dependence for Financial Time-Series

Assessing the predictive power of both data and models holds paramount significance in time-series machine learning applications. Yet, preparing time series data accurately and employing an appropriate measure for predictive power seems to be a non-trivial task. This work involves reviewing and establishing the groundwork for a comprehensive analysis of shaping time-series data and evaluating various measures of dependence. Lastly, we present a method, framework, and a concrete example for selecting and evaluating a suitable measure of dependence.

==> algorithm.tex <==
\begin{algorithmic}

\State
\State Initialize $W \gets 5$ \Comment{Sliding window size}
\State Initialize $N \gets 1$ \Comment{Sliding window step size}
\State Initialize $\lambda \gets r_{daily}$ \Comment{Target e.g. daily price return.}

\State
\State Initialize $b \gets 10$ \Comment{Bin Size}
\State Initialize matrix $D$ \Comment{Row-wise [features, target]}
\State Initialize vector $O$ \Comment{Correlation metric}

\State
\Repeat
\For{$i = 1, [w, \lambda, N, P]$} \Comment{Paramter search}
	\State Load time-series data $X$ from data source
	\For{$k = 1, K$} \Comment{Transform data}
	 	\State Compute return $R_k$ based on $\lambda$ and discretize with $b$
	 	\State Sample $X_k$ data from $X$ with width $w$	
	 	\State Create path $P_k$ (embedding) from $X_k$ \Comment{Or skip transformation}
	 	\State Compute signature $S_k$ from $P_k$
	 	\State Truncate signature terms that are  $len(S) > N$
	 	\State Transform signature to row vector $[S_k, R_k]$ with $N$ features 	
	 	\State Append row vector as feature columns to $D_k$
	\EndFor

	\State Apply multivariate non-linear correlation $D$ \Comment {Correlate data}
	\State Store correlation metric as order $O_i$  \Comment{i.g. MIC }
\EndFor

\State Find and store order with lowest value: \begin{center} $\Omega(w, \lambda) = \min O \leftarrow f(S(X_k \vert \mathbb{ I}^u_k))$
\end{center}

\Until{All test cases are completed}
\State Evaluate result matrix and find best result with highest $PP$ 
\State Done

\end{algorithmic}
